RoCap: A Robotic Data Collection Pipeline for the Pose Estimation of Appearance-Changing Objects

Object pose estimation plays a vital role in mixed-reality interactions when users manipulate tangible objects as controllers. Traditional vision-based object pose estimation methods leverage 3D reconstruction to synthesize training data. However, these methods are designed for static objects with diffuse colors and do not work well for objects that change their appearance during manipulation, such as deformable objects like plush toys, transparent objects like chemical flasks, reflective objects like metal pitchers, and articulated objects like scissors. To address this limitation, we propose Rocap, a robotic pipeline that emulates human manipulation of target objects while generating data labeled with ground truth pose information. The user first gives the target object to a robotic arm, and the system captures many pictures of the object in various 6D configurations. The system trains a model by using captured images and their ground truth pose information automatically calculated from the joint angles of the robotic arm. We showcase pose estimation for appearance-changing objects by training simple deep-learning models using the collected data and comparing the results with a model trained with synthetic data based on 3D reconstruction via quantitative and qualitative evaluation. The findings underscore the promising capabilities of Rocap.

==> contents/00.5_outline.tex <==
\section{Outline}

\begin{itemize}
    \item Intro (can Zhongyi write a draft first?) (\textbf{All authors})
    \item Related works
    \begin{itemize}
        \item Data collection method in HCI/CV (\textbf{Zhongyi \& Nick})
        \item learning-based pose estimation and state detection (existing dataset, custom dataset, few-shot) (\textbf{Zhongyi \& Toby})
    \end{itemize}
    \item Technical details
    \begin{itemize}
        \item Whole pipeline description 
        \item Data collection pipeline (\textbf{Nick})
        \begin{description}
            \item[] Robotic path planning
            \item[] change of state
            \item[] Image processing
            \item[] data augmentation for pose / segmentation
        \end{description}
        \item Training pipeline
        \begin{description}
            \item[Segmetation] MMdetection (\textbf{Nick})
            \item[Classification] (\textbf{Zhongyi})
            \item[Pose estimation] orientation and translation, maybe also state value regression? (\textbf{Toby})   
        \end{description}
    \end{itemize}
    \item Applications (\textbf{Toby})
    \begin{itemize}
        \item \textbf{Unconventional object tracking}: demonstrate tracking with unconventional object such as Tweezer (glossy and reflective), toy (very deformable)
        \item \textbf{object with different States}: A stupid punchable button which could launch a rocket; a scissor/clamp which will change the 
        \item \textbf{pose aware rendering}: place a \zhongyi{}{We need to highlight this aspect in writing. This is really something that make our work differ from others}
    \end{itemize}
    \item Evaluation
    \begin{description}
        \item[Expert interview?]
        \item[User study of a small number? (2-3 users)]  
    \end{description}

\end{itemize}

\subsection{Notes}

We will not invent our own neural network or we will largely build on existing work.

Some of the examples we could follow:
useful link: https://paperswithcode.com/task/6d-pose-estimation
\begin{itemize}
    \item PoseCNN \cite{xiang2017posecnn}
\end{itemize}


\subsection{Evaluation}


Some questions we need to answer:
\begin{itemize}
    \item Hand placement? is there only one position/configuration, we could use the AHAP in \cite{llop2019anthropomorphic} for our hand placement
    \item do we focus on only object dataset or object+hand dataset as in \cite{hampali2020honnotate}
    \item what are the representative of our rotation? quanternions or axis angle representation for the rotation?
    \item 
\end{itemize}

We could evaluate our system by:

\begin{itemize}
    \item Comparing the time of annotating a single object with the manual approach
    \item Whether the dataset generated by our system can work well with the existing CNN models
    \item test different types of objects: texture-ful, texture-less, multistates, etc
\end{itemize}

==> contents/05_Evaluation.tex <==
% \subsection{User Evaluation}

% \nick{explain a bit about how we processed the data for gen6d @Toby}
% We compare 


% \paragraph{MTurk}
% \nick{@Zhongyi, please update this paragraph}
% \subsection{User Evaluation}

\section{Evaluation}
% \nick{we shouldn't make it a whole section, the contribution is very limited.}
% \zhongyi{}{I still want to make it a whole session if we still have time. Evaluation is an important part of the paper. And we need to explain and justify why we choose these four objects in our studies and why we decide on this way to evaluate our system.}

People may question the need for using a robotic arm to perform data collection, as there is recent work focusing on pose estimation of physical objects with few-shot learning approaches \cite{sun2022onepose, liu2022gen6d, wen2023bundlesdf}. 
Typically, these methods require the input of a short video to reconstruct the 3D mesh of the objects \cite{sun2022onepose, liu2022gen6d} or a neural object field \cite{wen2023bundlesdf} to train on a small scale of data, 
and they have demonstrated competitive performance. 
However, similar to other prior work, these methods do not address the pose estimation of appearance-changing objects, which is an essential aspect of our focus. 
As a result, their performance may be limited when applied to objects with deformable properties, transparent materials, or multiple mechanical states. 
Therefore, to justify the needs of \codename{} and showcase its potential, we compared results with one of the few-shot learning method \cite{liu2022gen6d}. 

% In contrast, our robotic arm-based data collection approach effectively addresses these challenges for pose estimation of a wide variety of appearance-changing objects.

\subsection{Pose Estimation with Gen6D}
% To justify the needs and the potential of the \codename{} pipeline, we compared the results with another few-shot learning approach which does not require 
% To showcase the potential of the \codename{} pipeline, we compare the results with the few-shot approach that does not require the data collection process as people may have questioned. 

% To showcase the potential of the \codename{} pipeline, we compare its pose estimation results with a few-shot learning method \cite{liu2022gen6d} that does not require traditional data collection. Instead, Gen6D trains the model on a 3D mesh constructed from a short video of the objects.  

To perform 6D tracking using 3D reconstruction based tracking method~\cite{liu2022gen6d}, we followed the instruction from the authors and created 3D point cloud the object using a video with a moving camera pointing at the object. The resulting point cloud is then manually segmented to remove the background, and the orientation of the bounding box is manually specified. A detailed process of the data preparation can be found by their github page\footnote{https://github.com/liuyuan-pal/Gen6D}. 
The manual effort required both the method and \codename{} are similar with our method automating the capturing and segmentation process, but \codename{} requires longer unattended capturing time. We note that their method relies on 3D point cloud as a part of the input, therefore we could only use a single representative static state of the object when testing it.  
It also struggles to perform pose estimation on the set of appearance-changing objects as shown in Figure \ref{fig:results} bottom. 


Unlike methods trained on existing datasets, where the accuracy on the test set can be reported as a measure of improvement, there is no direct quantitative comparison between the two methods in this case.
Therefore, we recruited crowd workers to view and rate the performance of pose estimation in pairs of videos as a way to evaluate our approach.

% as a way to prove the improvements. 


\subsection{Crowd Worker Evaluation}

We recruited 50 crowd workers on Prolific\footnote{https://www.prolific.co/} and each of them viewed the pairs of videos for the four objects (Figure \ref{fig:results}) and rate the performance of pose estimation in a 5-point Likert-based question (1: L (left) is much worse than R (right), 2: L is slightly better than R, 3: the same, 4: L is slightly worse than R, 5: L is much better than R). 
We developed an HTML/JavaScript script to randomly swap the order of video pairs and converted the scores that higher scores signify better performance for \codename{}.
% We wrote a script of HTML/JavaScript to randomly swap the orders the pairs of video and convert the scores in a way that higher score sigifies the better performance of \codename{}.
Each crowd worker was paid 0.75 Pound.
% A refers to the video of using \codename{} and B refers to the video of using Gen6D. 

% To assess which model performs better pose estimation, we recruited crowd workers to vote for the better one. 
% For each video pair of the appearance-changing objects as shown in Figure \ref{fig:results} (i.e., \textit{video A} for the model trained on our data and \textit{video B} for Gen6D), 50 crowd workers assess the performance using a 1-5 Likert-based question (1: A is much worse than B, 2: A is slightly better than B, 3: the same, 4: A is slightly worse than B, 5: A is much better than B). 
% We randomly swap the order for the 
% \zhongyi{}{Should we also mention we randomly swap the left and right videos?}

% The results show that the pose estimation performance of model that is trained on data collected by \codename{} is much better than that of Gen6D. 
The ratings for the video pairs indicate that the estimation performance of the model trained on data collected by \codename{} is significantly better than that of Gen6D for appearance-changing objects (higher score signifies superior performance): Plushy toy (mean=4.20, $\sigma$=1.17), flask (mean=4.3, $\sigma$=1.10), clamp (mean=4.08, $\sigma$=1.15), and spray head (mean=4.12, $\sigma$=1.01). This demonstrates the potential of \codename{} in effectively handling appearance-changing objects.
% \nick{@Zhongyi fill in here}
% \paragraph{Study Design}
% \zhongyi{}{Add one or two paragraphs that justify why we choose these four objects}


% \subsection{Procedure}



% \subsection{Participants}

% \subsection{Results}

==> contents/99_outdated.tex <==
\section{Applications}

\nick{I will summarize application categories here}
Overall we need to support two types of applications, one requires rendering and the other one does not. 


We need to refer to sketch reality and create a overview figure of different applications here.
\subsection{Unconventional object tracking}
\zhongyi{}{needs to think about a better title}

\subsection{Object with Different States}

\subsection{Pose-aware Rendering}
\zhongyi{}{I recommend we should emphasize this aspect}


\section{Objects}
\nick{we need to have a clear plan of what kind of object we want to implement}

By default, we will assume that for all the objects, we could achieve 7DoF (6D Pose + State estimation).
However, some objects may not have states, some object may be too hard to estimate the 3D orientation.
So we will achieve 3D translation estimation for all object,
and whether we can estimate the 3D orientation and 1D state is depending on the characteristics of the object.

in the paper we will have a table to show case all the objects

Our target objects could be categorized as follows:
\begin{itemize}
    \item Conventional objects (rigid and easy to 3d reconstruct)
    \begin{itemize}
        \item rigid objects (No states)
        \begin{description}
            \item[Screwdriver:] application? 
            \item[Tiger:] render a speech bubble near the tiger. while 
        \end{description}
        \item objects with states
        \begin{itemize}
            \item Binary States
            \begin{description}
                \item[Button:] 
            \end{description}
            \item Continuous changing States
            \begin{description}
                \item[Clamp:] ideally the  
            \end{description}
            \item User customized states
            \begin{description}
                \item[Plush toy:] for example, a character from a seasame street, the user could capture two different states, one with the mouse open and one with the mouse closed. Then in the application, the action of closing the mouse will stop the audio for example.
            \end{description}
        \end{itemize}
    \end{itemize}
    \item Unconventional objects
    \begin{itemize}
        \item Deformable object 
        \begin{description}
            \item[Deformable toy:] what can we do using this type of plush toy?
        \end{description}
        \item Glossy / Reflective object
        \begin{description}
            \item[Tweezer:] 
        \end{description}
        \item Transparent
        \begin{description}
            \item[A coffee cup or bottle:] 
        \end{description}
    \end{itemize}
\end{itemize}
